MoEC: Mixture of Experts Implicit Neural Compression

Emerging Implicit Neural Representation (INR) is a promising data compression technique, which represents the data using the parameters of a Deep Neural Network (DNN). Existing methods manually partition a complex scene into local regions and overfit the INRs into those regions. However, manually designing the partition scheme for a complex scene is very challenging and fails to jointly learn the partition and INRs. To solve the problem, we propose MoEC, a novel implicit neural compression method based on the theory of mixture of experts. Specifically, we use a gating network to automatically assign a specific INR to a 3D point in the scene. The gating network is trained jointly with the INRs of different local regions. Compared with block-wise and tree-structured partitions, our learnable partition can adaptively find the optimal partition in an end-to-end manner. We conduct detailed experiments on massive and diverse biomedical data to demonstrate the advantages of MoEC against existing approaches. In most of experiment settings, we have achieved state-of-the-art results. Especially in cases of extreme compression ratios, such as 6000x, we are able to uphold the PSNR of 48.16.

==> table/abalation.tex <==
\begin{table}
  \caption{Ablation study}
  \label{table:ablatin}
  \centering
  \begin{tabular}{llll}
    \toprule
         & PSNR     & SSIM     \\
    \midrule
    Top-2     &51.59      &0.9937   \\
    w/o loss    &51.29       &0.9934   & \\
    Experts - 3    &\textbf{51.66}     &\textbf{0.9938} & \\
    Experts - 4    &51.40   &0.9935  & \\
    Top-2(1w epoch) &50.45 &0.9936 & \\
    \midrule
    \midrule
    MoEC    &51.56     &0.9931 & \\
    \bottomrule
  \end{tabular}
\end{table}


==> table/main.result.tex <==
%%%%%%%%%%%%%%%%%%%%%%    Baseline图     %%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figure/compare.png}
\caption{Visual comparisons with other benchmark method - 2D slices. We can observe that Other INR methods such as siren and nerf all suffer from ghosting artifacts. Our visual reconstruction effect is also better than traditional compression methods like SSF, h.264 and h.265.}
\vspace{-3mm}
\label{fig:decompress}
\end{figure*}



\begin{table*}[ht]
\caption{The average metrics on each dataset as compression ratio ranges from 64 to 256}

\renewcommand{\arraystretch}{1.0}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lllllllll}

\hline
           & \multicolumn{2}{c}{Lung} & \multicolumn{2}{c}{Heart} & \multicolumn{2}{c}{Kidney} & \multicolumn{2}{c}{Brain} \\ \cline{2-9} 
Methods    & PSNR        & SSIM       & PSNR        & SSIM        & PSNR         & SSIM        & PSNR        & SSIM        \\ \hline
MoEC(Ours) &43.54             &0.9503            &53.60             &\textbf{0.9949}             &47.56              &0.9815             &\textbf{50.27}             &\textbf{0.9861}             \\ \hline
JPEG       &    41.85    &   0.9650   &      46.68  &  0.9869     &   43.96      &  0.9690     &   42.315     &   0.9650          \\ \hline
H.264      &    44.93    &    0.9685  &  \textbf{56.37}      & 0.9901      &        \textbf{47.96} &  \textbf{0.9838}     &    49.36    &  0.9888     \\ \hline
HEVC       &   44.78     &  0.9680    &     53.67   & 0.9968      &   47.47      &  0.9828     &    48.64    &  0.9875     \\ \hline
SIREN      &  \textbf{43.96}      &  0.9598    &    53.14    &    0.9971   &      47.88   & 0.9835      &    48.47     & 0.9877      \\ \hline
NeRF       &    42.81    &   0.9522   &   49.20     &  0.9924     &   46.88      &  0.9800     &    47.00    &     0.9819        \\ \hline
NeRV       &   42.95     &   0.9540    &  49.86      &  0.9942     &  45.95       &    0.978    &    45.01    &  0.9753       \\ \hline
DVC        &   42.47     &   0.9531   &   46.95     &   0.9902    &   44.76      &   0.9723    &    44.32    &  0.9710           \\ \hline
SSF        &   45.04     &   \textbf{0.9699}   &  51.14      &   0.9953    &     47.17    & 0.9819      &    47.65    & 0.9849       \\ \hline
\end{tabular}
}
\label{table:main}
\end{table*}
